Optimal tie-breaking rules

We consider two-player contests with the possibility of ties and study the effect of different tie-breaking rules on effort. For ratio-form and difference-form contests that admit pure-strategy Nash equilibrium, we find that the effort of both players is monotone decreasing in the probability that ties are broken in favor of the stronger player. Thus, the effort-maximizing tie-breaking rule commits to breaking ties in favor of the weaker agent. With symmetric agents, we find that the equilibrium is generally symmetric and independent of the tie-breaking rule. We also study the design of random tie-breaking rules that are ex-ante fair and identify sufficient conditions under which breaking ties before the contest actually leads to greater expected effort than the more commonly observed practice of breaking ties after the contest.

==> final/rough.tex <==
\section{Literature review}

In this section, we collect the results that will be useful in our analysis.

\begin{lem}[\citet{fu2020optimal}]
\label{concave}
Let $C$ be a contest. Suppose there exist impact functions $f_i:\mathbb{R}_+ \to \mathbb{R}_+$ so that $P_i=\dfrac{f_i(x_i)}{f_1(x_1)+f_2(x_2)}$ for all $x_1,x_2 \geq 0$. If $f_i'(x_i)>0, f_i''(x_i)\leq 0$ for all $x_i \geq 0$, then there exists a unique pure strategy Nash equilibrium.
\end{lem}

Given the uniqueness, it is not hard to argue that the equilibrium effort level $x_i^*$ is either $0$ or it satisfies the first order condition. 
\citet{fu2020optimal} show that if the impact functions take the form $f_i(x_i)=\alpha_i h(x_i)+\beta_i$ and the designer's utility is increasing in effort, it can without loss of generality set all the headstarts $\beta_i=0$ and focus on optimally choosing the multiplicative biases $\alpha_i$. This result will be useful to us in our discussion of the \citet{blavatskyy2010contest} contest. 

% \citet{franke2018optimal} consider separately the problem of finding optimal biases and optimal headstarts in the lottery contest with impact functions $f_i(x_i)=\alpha_ix_i+\beta_i$. They show that with symmetric biases $\alpha_i=1$, the optimal headstarts depend on the discrepancy between the valuations of the two players. In particular, if $V_1 \geq 4V_2$, then the optimal headstart takes the form $(0,\frac{V_1}{4})$. And if $V_1 \leq 3V_2$, zero head starts are uniquely optimal. 

\begin{lem}[\citet{nti1999rent}]
\label{tullock}
Let $C$ be a contest such that $p_1=\frac{x_1^r}{x_1^r+x_2^r}$, $p_2=\frac{x_2^r}{x_1^r+x_2^r}$, $p_0=0$ and $c(x)=x$. If $r\leq 1$, then there exists a unique pure strategy Nash equilibrium and it is given by 
$$x_1^*= rV_1\dfrac{\beta^r}{(\beta^r+1)^2} \quad x_2^*=rV_2\dfrac{\beta^r}{(\beta^r+1)^2}$$
where $\beta=\dfrac{V_1}{V_2}$.
\end{lem}

\begin{lem}[\citet{baik2004two}]
\label{ratio}
Let $C=(V_1,V_2,p_1,p_2,q)$ be a contest. Suppose there exists a function $f:\mathbb{R}_+ \to \mathbb{R}_+$ so that $P_1=f(\theta)$ and $P_2=1-f(\theta)$ where $\theta=\frac{x_1}{x_2}$ for all $x_1,x_2 >0$. If $f'(\theta)>0, f''(\theta)<0$ and $2f'(\theta)+\theta f''(\theta)>0$ for all $\theta > 0$, then there exists a unique pure strategy Nash equilibrium and it is given by
$$x_1^*= V_1 \beta f'(\beta) \quad x_2^*=V_2 \beta f'(\beta)$$
where $\beta=\dfrac{V_1}{V_2}$.
\end{lem}


In the special case where the contest is symmetric and anonymous, \citet{malueg2006equilibria} identifies some simpler conditions under which a symmetric equilibrium exists and is unique.
\begin{lem}[\citet{malueg2006equilibria}]
\label{symmetric}
Let $C=(V,V,p_1,p_2,0.5)$ be a contest. Suppose there exists an increasing function $f:\mathbb{R}_+ \to \mathbb{R}_+$ so that $P_1=f(\theta)$ and $P_2=1-f(\theta)$ where $\theta=\frac{x_1}{x_2}$ for all $x_1,x_2 >0$ and $f$ satisfies $f(\theta)=1-f(\frac{1}{\theta})$ for all $\theta>0$. If $0<f'(1)\leq 0.5$ and $\exists \bar{\theta}$ such that $f''(\theta)<0$ for $\theta>\bar{\theta}$ and $\geq 0$ otherwise, then there is a unique symmetric pure strategy Nash equilibrium and it has both players exert effort $$x^*= Vf'(1)$$
\end{lem}

\section{Illustrative example}

The two-player lottery contest has been well-studied in the literature and takes the form $$p_i(x_i,x_{-i})=\dfrac{x_i}{x_1+x_2}$$ 
In this section, we will introduce the various ways in which contest success functions have been generalized to account for the possibility of ties through the lottery contest, and illustrate our results through these examples.

\subsection{\citet{blavatskyy2010contest}}

In this case, the contest success functions take the form
$$p_i(x_1,x_2)=\dfrac{x_i}{x_1+x_2+1}$$
Given a tie-breaking rule $q \in [0,1]$, the unique pure-strategy Nash equilibrium in the contest $C=(V_1,V_2,p_1(),p_2(),q)$ is  $$x_1^*=\frac{V_1^2 V_2}{\left(V_1+V_2\right)^2}-q \quad x_2^*=\frac{V_1 V_2^2}{\left(V_1+V_2\right)^2}-(1-q)$$


The tie-breaking rule $q \in [0,1]$ essentially defines different head-starts for the two players. There is a significant literature studying the design of optimal biased contests in which the designer is allowed to choose different head starts or multiplicative biases for the participants. In particular, \citet{fu2020optimal} showed that if the designer is able to control the multiplicative bias, it cannot gain from the ability to bias the contest using head-starts and so it may as well give no headstarts. \citet{franke2018optimal} shows that in two-player lottery contests with headstarts, it is optimal to give either no headstarts (if $v_1\leq 3v_2$) or a positive headstart to the weaker player (if $v_1 \geq 4v_2$).  Note that the general problem in our setup is different from these two problems. While these results suggest that headstarts generally discourage effort, in our case, the designer can only choose a distribution of a fixed budget of headstarts among the two players and cannot influence the budget. For the lottery contest in this example, the total effort remains the same irrespective of how the designer distributes this budget. We will see the more general and interesting analysis later.

\subsection{\citet{vesperoni2019contests}}

In this case, the contest success functions take the form
$$p_i(x_1,x_2)=\left(\dfrac{x_i}{x_1+x_2}\right)^2$$

Given a tie-breaking rule $q \in [0,1]$, the payoffs in the contest $C=(V_1,V_2,p_1(),p_2(),q)$ are  $$\Pi_1=V_1\left(\dfrac{x_1^2+2qx_1x_2}{(x_1+x_2)^2}\right)-x_1 \quad \Pi_2=V_2\left(\dfrac{x_2^2+2(1-q)x_1x_2}{(x_1+x_2)^2}\right)-x_2$$
Observe that in this case, the eventual contest success function $P_i(x_1,x_2)$ is homogeneous of degree $0$. Thus, we can write the contest success function more simply as a function of the ratio of efforts 
$\Pi_1=V_1p(\theta)-x_1 \quad \Pi_2=V_2(1-p(\theta))-x_2$
where $p(\theta)=\dfrac{\theta^2+2q\theta}{1+\theta^2+2\theta}$ and $\theta=\frac{x_1}{x_2}$.
This is the framework studied in \citet{baik2004two}.

Observe that $$p'(\theta)=\dfrac{2(q+\theta-q\theta)}{(\theta+1)^3}>0 \quad p''(\theta) =\frac{4 q(\theta-2)-4 \theta+2}{(\theta+1)^4} $$

\subsection{\citet{jia2012contests}}

In this case, the contest success functions take the form
$$p_i(x_1,x_2)=\left(\dfrac{x_i}{x_i+2x_{-i}}\right)$$


\subsection{Math facts}

\begin{lemrep}
The function $f: \mathbb{R}_+ \to \mathbb{R}$ defined by $f(x)=\dfrac{ax^2+bx}{(x+c)^2}-x$ is quasiconcave.
\end{lemrep}

\begin{proof}
We will show that the upper contour sets are convex. Take any $\alpha$ and suppose $x,y$ are such that $f(x) \geq \alpha, f(y) \geq \alpha$. We will show that $f(\frac{x}{2}+\frac{y}{2})\geq \alpha$. Because $f$ is continuous, this is sufficient to establish that the upper contour sets are convex.

We have that
$$\dfrac{ax^2+bx}{(x+c)^2} \geq x+\alpha \quad \dfrac{ay^2+by}{(y+c)^2} \geq y+\alpha$$

Taking the product, we get that
\begin{align*}
(x+\alpha)(y+\alpha)(x+c)^2(y+c)^2&\leq (ax^2+bx)(ay^2+by) \\
&= a^2x^2y^2+b^2xy+abxy(x+y)\\
&\leq a^2x^2y^2+b^2(x+y)^2/4+abxy(x+y)\\
&= \left(axy+b\left(\frac{x+y}{2}\right)\right)^2
\end{align*}

This implies $$\dfrac{2axy+bx+by}{2(x+c)(y+c)}\geq \sqrt{(x+\alpha)(y+\alpha))}$$


Now observe that 

\begin{align*}
f\left(\frac{x}{2}+\frac{y}{2}\right)&=\dfrac{a\left(\dfrac{x+y}{2}\right)^2+b\left(\dfrac{x+y}{2}\right)}{\left(\dfrac{x+y}{2}+c\right)^2}-\dfrac{(x+y)}{2}\\
&=\dfrac{ax^2+ay^2+2axy+2bx+2by}{(x+c)^2+(y+c)^2+2(x+c)(y+c)}-\dfrac{(x+y)}{2}\\
&=\dfrac{ax^2+bx+ay^2+by+2axy+bx+by}{(x+c)^2+(y+c)^2+2(x+c)(y+c)}-\dfrac{(x+y)}{2}\\
\end{align*}
\end{proof}


\section{Results}

In this section, we discuss our results.  We first consider a contest where the agents are ex-ante symmetric. In this setting, we identify natural sufficient conditions under which the contest game admits a symmetric Nash equilibrium that does not depend on the designer's choice of $v_0$. Hence, in these settings, the designer does not gain from introducing heterogeneity though $v_0$ in the contest. Later on, we consider a contest with asymmetric agents and show how the designer is better off if it runs a fair tie-break before the contest instead of running it after the contest.

\subsection{Tullock contests with symmetric agents}
In this subsection, we impose the following additional assumptions on our model.
\begin{itemize}
\item The probability of draw is homogeneous of degree $0$ i.e. $f_0(\lambda e_1,\lambda e_2)=f_0( e_1, e_2)$. In addition, it is maximized when $e_1=e_2$ and thus, $\dfrac{\partial f_0(e_1,e_2)}{\partial e_i}\Bigr|_{\substack{e_1=e\\e_2=e}}=0$ for all $e$. 
\item Both agents have the same cost functions $c_1(e)=c_2(e)=c(e)$.


\end{itemize}


\begin{thmrep}
\label{thm:symmetric}
Suppose $e^*$ is such that 
$$\dfrac{\partial f_i(e_1, e_2)} {\partial e_i}\Bigr|_{\substack{e_1=e^*\\e_2=e^*}}=\dfrac{d c(e)}{de}\Bigr|_{\substack{e=e^*}}$$
Then, $(e^*, e^*)$ is a pure strategy Nash equilibrium of the contest for any $v_0 \in [0,1]$.
\end{thmrep}
\begin{proof}
Given a $v_0$, player $1$'s payoff is given by
$$f_1(e_1,e_2)+v_0f_0(e_1,e_2)-c_1(e_1)$$ and player $2$'s payoff is given by
$$f_2(e_1,e_2)+(1-v_0)f_0(e_1,e_2)-c_2(e_2)$$

Taking the first order condition for player $1$ gives
\begin{equation} \label{eq:1}
\dfrac{\partial f_1(e_1,e_2)}{\partial e_1}+v_0\dfrac{\partial f_0(e_1,e_2)}{\partial e_1}=\dfrac{d c_1(e_1)}{de_1}
\end{equation}

and for player $2$ gives
\begin{equation} \label{eq:2}
\dfrac{\partial f_2(e_1,e_2)}{\partial e_2}+(1-v_0)\dfrac{\partial f_0(e_1,e_2)}{\partial e_2}=\dfrac{d c_2(e_2)}{de_2}
\end{equation}

% Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

Solving these simultaneously will give us the Nash equilibrium $e_1^*(v_0),e_2^*(v_0)$.


Let $e^*$ be such that $$\dfrac{\partial f_1(e_1, e_2)} {\partial e_1}\Bigr|_{\substack{e_1=e^*\\e_2=e^*}}=\dfrac{d c_1(e_1)}{de_1}\Bigr|_{\substack{e_1=e^*}}$$

Then, $(e^*, e^*)$ is a Nash equilibrium of the contest for any $v_0$. This is because we already know that $\dfrac{\partial f_0(e_1,e_2)}{\partial e_i}\Bigr|_{\substack{e_1=e\\e_2=e}}=0$ for all $e$. 

\end{proof}


We'd like to note here that these assumptions are satisfied by some of the well-known models of Tullock contests that allow for the possibility of ties. These models include the contest success function $f_i(e_i,e_{-i})=\left(\frac{e_i}{e_i+e_{-i}}\right)^k$ with $k \geq 1$ which was proposed and axiomatized by \citet{vesperoni2019contests}. In this model, the probability of tie is $f_0(e_1,e_2)=1-\dfrac{e_1^k+e_2^k}{(e_1+e_2)^k}$ which is both homogeneous of degree $0$ and maximized whenever $e_1=e_2$. Assuming linear costs of effort $c(e)=e$, we get the following as a corollary of Theorem \ref{thm:symmetric}. 

\begin{corollary}
Suppose the contest success function is $f_i(e_i,e_{-i})=\left(\frac{e_i}{e_i+e_{-i}}\right)^k$ with $k \geq 1$ and agents have linear costs $c(e)=e$. Then, there is a symmetric equilibrium such that $$e_1^*(v_0)=e_2^*(v_0)=\dfrac{k}{2^{k+1}}$$ for all $v_0$.
\end{corollary}


Another version of the Tullock contests that allows for ties is given by the contest success function $f_i(e_i,e_{-i})=\dfrac{e_i}{e_i+ke_{-i}}$ where $k \geq 1$. This model was axiomatized and proposed by \citet{jia2012contests}. Again, the probability of a tie in this model is $f_0(e_1,e_2)=1-\dfrac{e_1}{e_1+ke_2}-\dfrac{e_2}{e_2+ke_1}$ which is homogeneous of degree $0$ and is maximized when $e_1=e_2$. Assuming linear costs $c(e)=e$, we get another corollary of Theorem $\ref{thm:symmetric}$. 

\begin{corollary}
Suppose the contest success function is $f_i(e_i,e_{-i})=\dfrac{e_i}{e_i+ke_{-i}}$ with $k \geq 1$ and agents have linear costs $c(e)=e$. Then, there is a symmetric equilibrium such that $$e_1^*(v_0)=e_2^*(v_0)=\frac{k}{(1+k)^2}$$      for all $v_0$.
\end{corollary}

We conclude this section with a discussion of another generalization of Tullock contest with ties that does not satisfy our assumptions. In this model, the contest success function is given by $f_i(e_i,e_{-i})=\dfrac{e_i}{k+e_i+e_{-i}}$ where $k \geq 0$. This model was proposed by \citet{blavatskyy2010contest}. The probability of a draw is $f_0(e_1,e_2)=\dfrac{k}{k+e_1+e_2}$ which is not homogeneous of degree $0$ and the probability is always decreasing in effort. Therefore, theorem \ref{thm:symmetric} does not apply in this case. So we solve the model explicitly and find that even though the equilibrium itself depends on $v_0$, the total effort is again independent of choice of $v_0$. 

\begin{lemrep}
\label{thm:effort3}
Suppose the contest success function is $f_i(e_i,e_{-i})=\dfrac{e_i}{k+e_i+e_{-i}}$ with $k \geq 0$ and agents have linear costs $c(e)=e$. The equilibrium effort is given by $$e_1^*(v_0)=\frac{1}{4}-kv_0 \quad e_2^*(v_0)=\frac{1}{4}-k(1-v_0)$$ 
\end{lemrep}
\begin{proof}
Given a $v_0$, player $1$'s payoff is given by
$$(1-v_0)\dfrac{e_1}{k+e_1+e_2}+v_0\left(1-\dfrac{e_2}{k+e_1+e_2}\right)-e_1$$ and player $2$'s payoff is given by
$$v_0\dfrac{e_2}{k+e_1+e_2}+(1-v_0)\left(1-\dfrac{e_1}{k+e_1+e_2}\right)-e_2$$

Taking the first order condition for player $1$ gives
$$(1-v_0)\dfrac{k+e_2}{(k+e_1+e_2)^2} +v_0\dfrac{e_2}{(k+e_1+e_2)^2} =1$$
and for player $2$ gives
$$v_0\dfrac{k+e_1}{(k+e_1+e_2)^2} +(1-v_0)\dfrac{e_1}{(k+e_1+e_2)^2} =1$$

% Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

Solving, we get that the pure strategy Nash equilibrium takes the form:

$$e_1^*(v_0)=\frac{1}{4}-kv_0 \quad e_2^*(v_0)=\frac{1}{4}-k(1-v_0)$$ 
Then, the total effort under any $v_0$ is given by:
$$\frac{1}{2}-k$$



\end{proof}



\subsection{Single-shot contest}

In this subsection, we consider an instance of our model where
\begin{itemize}

\item $c(x)=x^2$ 
\item $p_i(x_i,x_{-i})=x_i(1-x_{-i})$
\end{itemize}

This resembles a setting where the agents get a single shot at a Basketball hoop and they can expend effort $x_i^2$ to better their probability $x_i$ of getting the shot. Player $i$ wins the contest if it is the only player to make the shot. The contest is drawn if both players make or miss the shot. 

\begin{thmrep}
In a single-shot contest, running a fair tie-breaker before the contest maximizes total effort among all ex-ante fair tie-breaking rules.    
\end{thmrep}


\begin{proof}
%tbd
\end{proof}

To prove the result, we first solve for the Nash equilibrium of the game for any fixed $v_0$. The following lemma notes the total effort in a Nash equilibrium of this game. 
\begin{lemrep}
\label{lem:effort1}
Given $v_0=\dfrac{1+\epsilon}{2}$, the total effort in the single-shot contest is given by 
$$e_1^*(\epsilon)+e_2^*(\epsilon)=\dfrac{\epsilon(c_1-c_2)+c_1+c_2+\epsilon^2}{4c_1c_2+\epsilon^2}.$$
\end{lemrep}

\begin{proof}
Given a $v_0$, player $1$'s payoff is given by
$$e_1(1-e_2)+v_0\left(e_1e_2+(1-e_1)(1-e_2)\right)-c_1e_1^2$$ and player $2$'s payoff is given by
$$e_2(1-e_1)+(1-v_0)\left(e_1e_2+(1-e_1)(1-e_2)\right)-c_2e_2^2$$

Taking the first order condition for player $1$ gives
$$1-e_2+v_0e_2-v_o(1-e_2)-2c_1e_1=0 \iff e_1=\dfrac{(1-v_0)(1-e_2)+v_0e_2}{2c_1}$$
and for player $2$ gives
$$1-e_1+(1-v_0)(e_1-(1-e_1))-2c_2e_2=0 \iff e_2=\dfrac{v_0(1-e_1)+(1-v_0)e_1}{2c_2}$$

% Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

Solving, we get that the pure strategy Nash equilibrium takes the form:
$$e_1^*(v_0)= \dfrac{(2v_0-1)v_0+2c_2(1-v_0)}{4c_1c_2+(1-2v_0)^2} \quad e_2^*(v_0)=\dfrac{(1-2v_0)(1-v_0)+2c_1v_0}{4c_1c_2+(1-2v_0)^2}$$

Then, the total effort under any $v_0$ is given by:

$$e_1^*(v_0)+e_2^*(v_0)=\dfrac{2v_0(c_1-c_2)+2c_2+(1-2v_0)^2}{4c_1c_2+(1-2v_0)^2}$$

Let $v_0=\frac{1+\epsilon}{2}$. Then, we can rewrite the total effort as 
$$e_1^*(\epsilon)+e_2^*(\epsilon)=\dfrac{\epsilon(c_1-c_2)+c_1+c_2+\epsilon^2}{4c_1c_2+\epsilon^2}$$

In the special case where both players are symmetric so that $c_1=c_2=c$, the total effort is 
$$\dfrac{2c+\epsilon^2}{4c^2+\epsilon^2}$$
Differentiating with respect to $\epsilon$, we get
$$\dfrac{2\epsilon(2c)(2c-1)}{\left(4c^2+\epsilon^2\right)^2}$$

Observe that the total effort is symmetric around $\epsilon=0$ and in addition, it is decreasing for $\epsilon<0$ and increasing after $\epsilon>0$ (because $c>\frac{1}{2}$). Thus, the designer prefers to set either $\epsilon=1$ ($v_0=1$) or $\epsilon=-1$ ($v_0=0$) to maximize total effort and is indifferent between the two choices. When it must be fair to both players, it can toss a fair coin before the contest to determine the winner in case of a draw. So having the tie breaker before the contest leads to a greater amount of total effort when the players are symmetric. 



% Consider the special case where $c_1=1,c_2=\frac{1}{2}$. Then the total effort is given by $\dfrac{\epsilon+3+2\epsilon^2}{4+2\epsilon^2}$ and we can check that it is maximized at $\epsilon=1$. So, the designer would want to bias the contest in favor of the weaker agent to maximize total effort. But what if we require the designer to be ex-ante fair so that $\mathbb{E}[\epsilon]=0$? 

Now let's consider the general case and only compare the two scenarios i) toss after the contest and ii) toss before the contest. 
When toss is done after the contest so that $\epsilon=0$, the total effort is $\frac{c_1+c_2}{4c_1c_2}$ and when it is done before the contest, the total expected effort is 
$ \frac{c_1+c_2+1}{4c_1c_2+1}$

Since $c_1+c_2<4c_1c_2$, we get that the expected effort from having the toss before the contest dominates having the toss after the contest. 


% Now let's try to solve for the optimal tie-breaking rule when the designer is constrained to be ex-ante fair. 
% In the general case, the derivative of total effort takes the form:

% $$\dfrac{\left(4c_1c_2+\epsilon^2\right)(c_1-c_2+2\epsilon)-(\epsilon(c_1-c_2)+c_1+c_2+\epsilon^2)2\epsilon}{\left(4c_1c_2+\epsilon^2\right)^2}$$
% which equals
% $$\dfrac{-\epsilon^2(c_1-c_2)+2\epsilon(4c_1c_2-c_1-c_2)+(c_1-c_2)4c_1c_2}{\left(4c_1c_2+\epsilon^2\right)^2} $$

\end{proof}

When $c_1>c_2$, the total effort is increasing in $\epsilon$ and therefore, if the designer can afford to be biased, it will resolve ties in favor of the weaker player. 
\begin{corollary}
In a single-shot contest, if $c_1>c_2$, the optimal tie-breaking rule breaks ties in favor of player $1$ by setting $v_0=1$.
\end{corollary}

Now let's discuss the case where the designer must be unbiased.
Two simple unbiased tie-breaking rules are running a fair tie-breaker before or after the contest. The expected total effort from running the tie-breaker before the contest $(\epsilon=1,-1 \text{ with equal probability})$ equals $\dfrac{c_1+c_2+1}{4c_1c_2+1}$ while that from running the tie-breaker after the contest $(\epsilon=0)$ equals $\dfrac{c_1+c_2}{4c_1c_2}$. So we know that total expected effort from having a fair tie-breaker before the contest is always greater than that from having the tie-breaker after the contest. 

To prove the optimality of breaking the breaking ties before the contest among all fair tie-breaking rules, we first show that the support of the optimal distribution will be at most two points. And then, using the constraint on the expectation, we are able to express the problem as a single parameter optimization problem. 
The full proof is in the appendix.








\subsection{Geometric contest}

In this section, we consider an instance of our model where 
\begin{itemize}

\item $c_i(e_i)=c_ie_i$ with $c_i \geq \frac{1}{2}$
\item $f_i(e_i,e_{-i})= \dfrac{e_i-e_ie_{-i}}{e_i+e_{-i}-e_ie_{-i}}$. 
\end{itemize}

This resembles a setting where the agents get multiple shots at a Basketball hoop and they can expend effort $c_ie_i$ to better their probability $e_i$ of getting the shot. Player $i$ wins if it is the first player to make the shot. The contest is drawn if both players make their first shot after missing the same number of times. 

% \href{https://www.desmos.com/calculator/xcemrrxtla}{Desmos graph} illustrating equilibrium (the point of intersection of the two curves between $0$ and $1$) as a function of $v_0$.

\begin{thmrep}
\label{thm:effort2}
In a geometric contest with symmetric players and $\frac{1}{2} \leq c \leq \frac{2}{3}$, the total effort from running a tie-breaker after the contest is greater than that from running it before the contest.
\end{thmrep}

\begin{proof}
Given a $v_0$, player $1$'s payoff is given by
$$\dfrac{e_1-e_1e_2}{e_1+e_2-e_1e_2}+v_0\dfrac{e_1e_2}{e_1+e_2-e_1e_2}-c_1e_1$$ and player $2$'s payoff is given by
$$\dfrac{e_2-e_1e_2}{e_1+e_2-e_1e_2}+(1-v_0)\dfrac{e_1e_2}{e_1+e_2-e_1e_2}-c_2e_2$$

Taking the first order condition for player $1$ gives

$$\dfrac{(e_1+e_2-e_1e_2)(1-e_2+v_0e_2)-e_1(1-e_2+v_0e_2)(1-e_2)}{(e_1+e_2-e_1e_2)^2}=c_1$$
which simplifies to
$$\dfrac{(e_2)(1-(1-v_0)e_2)}{(e_1+e_2-e_1e_2)^2}=c_1$$


For player $2$, the foc gives
$$\dfrac{(e_1)(1-v_0e_1)}{(e_1+e_2-e_1e_2)^2}=c_2$$

% Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$


For $v_0=\frac{1}{2}$ and $c_1=c_2=c$, the symmetric NE is unique and is given by $(e^*,e^*)$ where 
$$e^*=1-\sqrt{1-\frac{1}{2c}}$$

Compare this to the case where a fair toss is executed before the contest. 

Let's say then $v_0=0$. In this case, the two foc conditions become 
$$\dfrac{e_2(1-e_2)}{(e_1+e_2-e_1e_2)^2}=c= \dfrac{e_1}{(e_1+e_2-e_1e_2)^2}$$

In particular, we have that $e_1=e_2(1-e_2)$ and thus, $e_1+e_2=e_2(2-e_2)$. 

Note that the maximum possible value of $e_2(2-e_2)$ is $1$. Thus, if $2-2\sqrt{1-\frac{1}{2c}} \geq 1 \iff c \leq \frac{2}{3}$, then the total effort from running the tie-break after the contest is greater than that from running it before the contest. Thus, we get that for $\frac{1}{2}\leq c \leq \frac{2}{3}$, it is better to run a fair tie-break after the contest than running it before the contest. 

% Observe that $e_2(2-e_2)$ is increasing in $e_2$ and is maximized at $e_2=1$, at which point the objective also takes the value $1$. If we can obtain a better upper bound on $e_2$, it will lead to a better upper bound on the value of the objective.

% From the foc, we have that 
% $$e_2(1-e_2)=c(e_2(2-e_2-e_1))^2$$ so that
% $$\dfrac{1-e_2}{ce_2}=(2-e_1-e_2)^2 \implies e_1+e_2=2-\sqrt{\dfrac{1-e_2}{ce_2}}$$
\end{proof}


Thus, in comparison to a single-shot contest where we showed that running tie-breaker before the contest was optimal among all fair tie-breaking rules, we see that the designer is better off running a fair tie-break after the agents have played in a geometric contest. We believe that the optimality of running a fair-tie break afterwards is optimal more generally but haven't been able to establish that.



% \subsection{Exponential contest}


% In this section, we consider an instance of our model where 
% \begin{itemize}

% \item $c_i(e_i)=c_ie_i$
% \item $f_i(e_i,e_{-i})= \dfrac{e_i}{e_i+e_{-i}}\exp({-e_{-i}\delta})$. 
% \end{itemize}

% This resembles a setting where the agents can invest effort cost $c_ie_i$ to improve their time to success which follows an exponential distribution with parameter $e_i$. An agent wins if it scores at least $\delta$ before the other agent. If the scores of the two agents are within $\delta$ of each other, the contest is considered a tie. 

% \begin{thmrep}

% \end{thmrep}

% \begin{proof}
% Given a $v_0$, player $1$'s payoff is given by
% $$(1-v_0)\dfrac{e_1}{e_1+e_2}\exp({-e_2\delta})+v_0\left(1-\dfrac{e_2}{e_1+e_2}\exp({-e_1\delta})\right)-c_1e_1$$ and player $2$'s payoff is given by
% $$v_0\dfrac{e_2}{e_1+e_2}\exp({-e_1}\delta)+(1-v_0)\left(1-\dfrac{e_1}{e_1+e_2}\exp({-e_2}\delta)\right)-c_2e_2$$




% \end{proof}


% \subsection{Example 5: All-pay auction with ties}

% In this subsection, we consider an instance of our model where 
% \begin{itemize}

% \item $c_i(e_i)=c_ie_i$
% \item $f_i(e_i,e_{-i})=\left\{\begin{array}{ll}
% 1 & \text { if } e_i-e_{-i} > k \\
% 0 & \text { if } e_i-e_{-i} \leq k\\
% \end{array}\right.$. 
% \end{itemize}

% This resembles an all-pay auction allowing for the possibility of ties (\citet{gelder2019all}). If $|e_i-e_{-i}| \leq k$, the contest is drawn and the tie-breaking rule kicks in. 










% \subsection{Example 2: Modified Tullock contest}

% In this subsection, we consider an instance of our model where 
% \begin{itemize}

% \item $c_i(e_i)=c_ie_i$
% \item $f_i(e_i,e_{-i})=\frac{e_i}{e_i+e_{-i}}*(1-d)$, 
% \end{itemize}

% This resembles a setting where there is a constant probability $d$ of the contest ending in a draw. This might be due to external factors like rain washing out the game etc which is independent of the effort exerted by the agents.  Note that with $d=0$, this would be a standard Tullock contest with discriminatory power $r=1$. 

% \begin{lemrep}
% \label{thm:effort2}
% Given $v_0$, the total effort in the modified Tullock contest is given by 
% $$e_1^*+e_2^*=\dfrac{1-d}{c_1+c_2}.$$
% \end{lemrep}

% \begin{proof}
% Given a $v_0$, player $1$'s payoff is given by
% $$\dfrac{e_1}{e_1+e_2}(1-d)+dv_0-c_1e_1$$ and player $2$'s payoff is given by
% $$\dfrac{e_2}{e_1+e_2}(1-d)+d(1-v_0)-c_2e_2$$

% Taking the first order condition for player $1$ gives
% $$\dfrac{e_2(1-d)}{(e_1+e_2)^2}-c_1=0  $$
% and for player $2$ gives
% $$\dfrac{e_1(1-d)}{(e_1+e_2)^2}-c_2=0  $$
% Taking the ratio gives $e_1c_1=e_2c_2$
% % Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

% Solving, we get that the pure strategy Nash equilibrium takes the form:
% $$e_1^*(v_0)= \dfrac{c_2(1-d)}{(c_1+c_2)^2} \quad e_2^*(v_0)=\dfrac{c_1(1-d)}{(c_1+c_2)^2}$$

% Then, the total effort under any $v_0$ is given by:

% $$e_1^*(v_0)+e_2^*(v_0)=\dfrac{1-d}{c_1+c_2}$$
% \end{proof}



% \subsection{Example 2: Modified Tullock contest 1}


% In this subsection, we consider an instance of our model where 
% \begin{itemize}

% \item $c_i(e_i)=e_i$
% \item $f_i(e_i,e_{-i})=\left(\frac{e_i}{e_i+e_{-i}}\right)^k$ where $k \geq 1$. 
% \end{itemize}

% This resembles modified version of Tullock contest allowing for the possibility of ties (\citet{vesperoni2019contests}). With $k=1$, this is a standard Tullock contest with discriminatory power $r=1$. 

% \begin{thmrep}
% \label{thm:effort2}
% Given $v_0$, the total effort in the Modified Tullock contest 1 is given by 
% $$e_1^*(v_0)+e_2^*(v_0)=\dfrac{k}{2^k}.$$ In fact, the equilibrium is such that $e_1^*(v_0)=e_2^*(v_0)=\dfrac{k}{2^{k+1}}$ for all $v_0$. 
% \end{thmrep}

% \begin{proof}
% Given a $v_0$, player $1$'s payoff is given by
% $$(1-v_0)\dfrac{e_1^k}{(e_1+e_2)^k}+v_0\left(1-\dfrac{e_2^k}{(e_1+e_2)^k}\right)-e_1$$ and player $2$'s payoff is given by
% $$v_0\dfrac{e_2^k}{(e_1+e_2)^k}+(1-v_0)\left(1-\dfrac{e_1^k}{(e_1+e_2)^k}\right)-e_2$$

% Taking the first order condition for player $1$ gives
% $$(1-v_0) k \left(\dfrac{e_1}{e_1+e_2}\right)^{k-1} \dfrac{e_2}{(e_1+e_2)^2}+v_0k\left(\dfrac{e_2}{e_1+e_2}\right)^{k-1}\dfrac{e_2}{(e_1+e_2)^2} =1$$
% and for player $2$ gives
% $$v_0 k \left(\dfrac{e_2}{e_1+e_2}\right)^{k-1} \dfrac{e_1}{(e_1+e_2)^2}+(1-v_0)k\left(\dfrac{e_1}{e_1+e_2}\right)^{k-1}\dfrac{e_1}{(e_1+e_2)^2} =1$$

% % Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

% Solving, we get that the pure strategy Nash equilibrium takes the form:
% $$e_1^*(v_0)=e_2^*(v_0)= \dfrac{k}{2^{k+1}}$$

% Then, the total effort under any $v_0$ is given by:

% $$e_1^*(v_0)+e_2^*(v_0)=\dfrac{k}{2^k}$$


% \end{proof}

% It is perhaps surprising that the equilibrium effort profile is symmetric and that it does not depend on $v_0$. To see why there exists such an equilibrium, observe that the modified Tullock contest is such that the probability of a draw is maximized whenever $e_i=e_{-i}$. It follows then that $\dfrac{\partial f_0(e_1,e_2))}{\partial e_i}=0$ whenever $e_1=e_2$. It follows from the characterization equations \ref{eq:1} and \ref{eq:2} then that there is a solution where $e_1=e_2=e$ which is independent of $v_0$. It turns out that this is the only equilibrium in this contest.  


% \subsection{Example 4: Modified Tullock 3}

% In this subsection, we consider an instance of our model where 


% \begin{itemize}

% \item $c_i(e_i)=e_i$
% \item $f_i(e_i,e_{-i})=\frac{e_i}{e_i+ke_{-i}}$ where $r \in (0,\infty)$ and $k \geq 1$. 
% \end{itemize}

% This resembles another modified version of Tullock contest allowing for the possibility of ties (\citet{jia2012contests}). With $k=1$, this is a standard Tullock contest with discriminatory power $r=1$. 


% \begin{thmrep}
% \label{thm:effort4}
% Given $v_0$, the total effort in the Modified Tullock contest 2 is given by 
% $$e_1^*(v_0)+e_2^*(v_0)=\frac{2k}{(1+k)^2}$$ In particular, the equilibrium effort is given by  $$e_1^*(v_0)=\frac{k}{(1+k)^2} \quad e_2^*(v_0)=\frac{k}{(1+k)^2}$$     
% \end{thmrep}
% \begin{proof}
% Given a $v_0$, player $1$'s payoff is given by
% $$(1-v_0)\dfrac{e_1}{e_1+ke_2}+v_0\left(1-\dfrac{e_2}{ke_1+e_2}\right)-e_1$$ and player $2$'s payoff is given by
% $$v_0\dfrac{e_2}{ke_1+e_2}+(1-v_0)\left(1-\dfrac{e_1}{e_1+ke_2}\right)-e_2$$

% Taking the first order condition for player $1$ gives
% $$(1-v_0)\dfrac{ke_2}{(e_1+ke_2)^2} +v_0k\dfrac{e_2}{(ke_1+e_2)^2} =1$$
% and for player $2$ gives
% $$v_0\dfrac{ke_1}{(ke_1+e_2)^2} +(1-v_0)k\dfrac{e_1}{(e_1+ke_2)^2} =1$$

% % Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

% Solving, we get a pure strategy Nash equilibrium:

% $$e_1^*(v_0)=\frac{k}{(1+k)^2} \quad e_2^*(v_0)=\frac{k}{(1+k)^2}$$ 
% Then, the total effort under any $v_0$ is given by:
% $$\frac{2k}{(1+k)^2}$$

% \end{proof}

% In this case again, observe that $$f_0(e_1,e_2)=1-\dfrac{e_1}{e_1+ke_2}-\frac{e_2}{ke_1+e_2}$$

% Taking the partial derivative with respect to $e_1$, we get
% $$\dfrac{\partial f_0(e_1,e_2)}{\partial e_1}=-\left(\dfrac{ke_2}{(e_1+ke_2)^2}-\dfrac{ke_2}{(ke_1+e_2)^2}\right)$$

% This again equals $0$ when $e_1=e_2$ and so we get that a symmetric equilibrium $e_1=e_2$ exists which is independent of $v_0$. 

% \subsection{Example 3: Modified Tullock 2}

% In this subsection, we consider an instance of our model where 
% \begin{itemize}

% \item $c_i(e_i)=e_i$
% \item $f_i(e_i,e_{-i})=\frac{e_i}{k+e_i+e_{-i}}$ where $k \geq 0$. 
% \end{itemize}

% This resembles another modified version of Tullock contest allowing for the possibility of ties (\citet{blavatskyy2010contest}). With $k=0$, this is a standard Tullock contest with discriminatory power $r=1$. 

% \begin{thmrep}
% \label{thm:effort3}
% Given $v_0$, the total effort in the Modified Tullock contest 2 is given by 
% $$e_1^*(v_0)+e_2^*(v_0)=\dfrac{1}{2}-k.$$ In particular, the equilibrium effort is given by  $$e_1^*(v_0)=\frac{1}{4}-kv_0 \quad e_2^*(v_0)=\frac{1}{4}-k(1-v_0)$$     
% \end{thmrep}
% \begin{proof}
% Given a $v_0$, player $1$'s payoff is given by
% $$(1-v_0)\dfrac{e_1}{k+e_1+e_2}+v_0\left(1-\dfrac{e_2}{k+e_1+e_2}\right)-e_1$$ and player $2$'s payoff is given by
% $$v_0\dfrac{e_2}{k+e_1+e_2}+(1-v_0)\left(1-\dfrac{e_1}{k+e_1+e_2}\right)-e_2$$

% Taking the first order condition for player $1$ gives
% $$(1-v_0)\dfrac{k+e_2}{(k+e_1+e_2)^2} +v_0\dfrac{e_2}{(k+e_1+e_2)^2} =1$$
% and for player $2$ gives
% $$v_0\dfrac{k+e_1}{(k+e_1+e_2)^2} +(1-v_0)\dfrac{e_1}{(k+e_1+e_2)^2} =1$$

% % Then $2c_1e_1+2c_2e_2=1+2v_0(e_2-e_1)$

% Solving, we get that the pure strategy Nash equilibrium takes the form:

% $$e_1^*(v_0)=\frac{1}{4}-kv_0 \quad e_2^*(v_0)=\frac{1}{4}-k(1-v_0)$$ 
% Then, the total effort under any $v_0$ is given by:
% $$\frac{1}{2}-k$$

% \end{proof}

% There is no one-size-fits-all answer to this question because the optimal tie-breaking rules will depend on the context in which they are being used. Some common tie-breaking methods include:

% Extra time or additional rounds: This is a common method used in sports tournaments and other competitive events where two or more participants tie. The competitors are given additional time or rounds to compete, and the winner is determined by their performance in these extra rounds.

% Sudden death: In this method, the competitors are given a specific task or challenge, and the first person to complete it wins the tie-break. This method is often used in sports like soccer, where the first team to score a goal in extra time wins the match.

% Coin toss: This is a simple and quick method of breaking a tie, where a coin is flipped to determine the winner. It is often used in games or situations where there is no time for a more complex tie-breaking method.

% Drawing lots: This method involves randomly selecting a winner from the pool of competitors who have tied. This can be done using a random number generator or by physically drawing names or numbers from a hat.

% Ultimately, the best tie-breaking method will depend on the specific situation and the preferences of the participants. It is important to clearly communicate the tie-breaking rules before the competition begins to ensure that everyone is aware of how ties will be resolved.

% \subsection{Poisson contest}

% In this section, we consider an instance of our model where 
% \begin{itemize}

% \item $c_i(e_i)=c_ie_i$ 
% \item $f_i(e_i,e_{-i})=\mathbb{P}[X(e_i) > X(e_{-i})]$ where $X(c)$ is Poisson with mean $c$. 
% \end{itemize}

% This resembles a setting where the agents output will be a Poisson random variable and they can expend effort $c_ie_i$ to better their mean score $e_i$. Player $i$ wins if it scores more than the other agent. The contest is drawn if both players have the same score. This contest was considered in \citet{keller1994characterization}.


\section{Difference-form contest success functions}

In this section, we consider instances of our model where the distribution over the three outcomes depends only on  the difference of the efforts $\theta=x_1-x_2$ of the two players. Formally, we assume that there exist functions $p:\mathbb{R}\to [0,1]$ and $p_0:\mathbb{R}\to [0,1]$ such that
\begin{itemize}
    \item $p_1(x_1, x_2)=p(\theta)$ and $p_2(x_1,x_2)=p(-\theta)$
    \item $p_0(x_1, x_2)=p_0(\theta)$ and $p_0(\theta)=p_0(-\theta)$ for all $\theta \in \mathbb{R}_+$
    \item $c(x)=x$
\end{itemize}


We'll make the following assumption on these functions.

\begin{assumption}
\label{ass:existence}
Suppose $z_q(\theta)=p(\theta)+qp_0(\theta)$. For any $q\in [0,1]$,  $z_q^{\prime}(\theta)>0, z_q^{\prime \prime}(\theta)<0$, and $2 z_q^{\prime}(\theta)+\theta z_q^{\prime \prime}(\theta)>0$, for all $\theta$ in $R_{+}$.
\end{assumption}

Note that $z_q(\theta)$ denotes the probability that player $1$ eventually wins the prize and $1-z_q(\theta)$ is the probability that player $2$ wins eventually wins the prize. The assumption then says that a player's probability of winning is increasing in its own effort, decreasing in the effort of the other player, and in addition, it is increasing at a decreasing rate in one's own effort. 

The next assumption we make is on the probability of ties $p_0(\theta)$ and is motivated by the idea that the probability of a tie increases as the contest becomes more closely contested. 

\begin{assumption}
\label{ass:tie}
The probability of tie $p_0(\theta)$ is increasing for $\theta \in (0,1]$ and decreasing for $\theta \in [1, \infty)$. 
\end{assumption}

% @inproceedings{kleinberg2011mechanisms,
%   title={Mechanisms for (mis) allocating scientific credit},
%   author={Kleinberg, Jon and Oren, Sigal},
%   booktitle={Proceedings of the forty-third annual ACM symposium on Theory of computing},
%   pages={529--538},
%   year={2011}
% }

% @article{konrad2009multi,
%   title={Multi-battle contests},
%   author={Konrad, Kai A and Kovenock, Dan},
%   journal={Games and Economic Behavior},
%   volume={66},
%   number={1},
%   pages={256--274},
%   year={2009},
%   publisher={Elsevier}
% }

% @article{keller1994characterization,
%   title={A characterization of the Poisson distribution and the probability of winning a game},
%   author={Keller, Joseph B},
%   journal={The American Statistician},
%   volume={48},
%   number={4},
%   pages={294--298},
%   year={1994},
%   publisher={Taylor \& Francis}
% }

% @article{harris1987racing,
%   title={Racing with uncertainty},
%   author={Harris, Christopher and Vickers, John},
%   journal={The Review of Economic Studies},
%   volume={54},
%   number={1},
%   pages={1--21},
%   year={1987},
%   publisher={Wiley-Blackwell}
% }

